Multi-fidelity Gaussian process surrogate modeling for regression problems in physics

One of the main challenges in surrogate modeling is the limited availability of data due to resource constraints associated with computationally expensive simulations. Multi-fidelity methods provide a solution by chaining models in a hierarchy with increasing fidelity, associated with lower error, but increasing cost. In this paper, we compare different multi-fidelity methods employed in constructing Gaussian process surrogates for regression. Non-linear autoregressive methods in the existing literature are primarily confined to two-fidelity models, and we extend these methods to handle more than two levels of fidelity. Additionally, we propose enhancements for an existing method incorporating delay terms by introducing a structured kernel. We demonstrate the performance of these methods across various academic and real-world scenarios. Our findings reveal that multi-fidelity methods generally have a smaller prediction error for the same computational cost as compared to the single-fidelity method, although their effectiveness varies across different scenarios.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}

==> sections/theory/mf_gaussian.tex <==
Multi-fidelity could be realized by introducing a prior (in the case of Bayesian modeling). In the Gaussian process, the prior is set by a kernel, therefore a kernel could be constructed in a way that utilizes lower-fidelity functions. Kernel emulates the covariance in GP, so with the advantage of the lower-fidelity function we can come closer to the "real" covariance between the HF data points, using a similarity measure derived from the lower-fidelity functions. 
For example, if we take a derivative of a lower-fid function in point x and in point y, and if their derivatives are close enough ("closeness is measured via dot prod, for example), then we have a reason to speculate, that the behavior of HF function in points x and y will have the same similarity, as similarity in behavior of lower-fidelity function in this point.
This will be still a valid kernel, while the outsputs of dot-product are always positive semi-definite. 
\begin{equation}
    K(x, x^{*}) = <f_{lofi}(x), f_{lofi}(x^{*})>
\end{equation}
Another approach inspired by the GP construction with the coefficient being the Gaussian process itself... (?) \cite{le2013multi}. To capture the connection between the lofi and hifi, could be utilized analogue co-Kriging (=multi-output GP)... Actual coKriging consider only linear correlation between the functions, therefore couldn't be efficiently used. But by defining $f_l$ as a samples from $u_l$, where $u_l ~ N(0, K_{ll})$ we can model a hifi function in the next way: $f_h = u_l(1+u_p) + u_s$. And the scaling factor $u_p$ could be represented here by another GP. Therefore...

Proof that kernel of this thing will still be a legit kernel: ...
